Towards an executable semantics of automobile RTOS standard and its application to conformance verification

The automobile Real-Time Operating System (RTOS) is hard to design and implement due to its real time features and increasing complexity. Some automobile RTOS standards are released aiming at unifying the software architecture of vehicle systems. Most of the standards are presented informally in natural languages, which may lead to not only ambiguities in specifications but also difficulties in conformance verification. This paper proposes a rewriting-based approach for formalising the automobile RTOS standard. Taking the OSEK/VDX standard as an example, an executional formal semantics of the automobile RTOS kernel, which focuses on the real time features, is defined using $\mathbb{K}$, a rewriting-based framework. We also report some ambiguous definitions of the OSEK/VDX standard, which we find in the process of formalisation. The $\mathbb{K}$ semantics of the OSEK/VDX standard is applied to conformance verification, which is used to check the conformance of not only the automobile operating system kernel but the applications.

==> abstract.tex <==
%\footnotetext[1]{Corresponding author}
\begin{abstract}
Due to its strong timeliness and maintainability, real time operating system (RTOS) has been applied in various of safety-critical systems, such as in the vehicle systems. Some automobile RTOS standards are released for the reason of unifying the software architecture of vehicle systems. The standards presented in natural languages may lead misunderstandings. This paper propose a semantic-based  approach for formalizing the automobile RTOS standard. Taking OSEK/VDX standard as example, an executional formal semantics of the automobile RTOS kernel, which depicts the real time features, is defined using K framework. To demonstrate the usefulness of the proposed approach, an industrial application specified with OSEK/VDX standard is analyzed and verified under the formal semantics. 
%This work shows real time features of RTOS can be 
\end{abstract}

==> commands_packages.tex <==
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb,epsfig,amstext,graphics}
\usepackage{times}
\usepackage{indentfirst}
\usepackage{mcite}
\usepackage{wasysym}
\usepackage{booktabs}
\usepackage{stmaryrd}
\usepackage{mathrsfs}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{listings}
\lstset{numbers=left,
  numberstyle=\scriptsize,
  keywordstyle=\color{blue!70},
  commentstyle=\color{red!50!green!50!blue!50},
  frame=none,
  flexiblecolumns=false,
  language=C,
  basicstyle=\ttfamily\small,
  breaklines=true,
  extendedchars=true,
  escapechar=\%,
  texcl=true,
  showstringspaces=true,
 % keywordstyle=\bfseries,
  tabsize=4}
\usepackage{setspace}
\let\proof\relax
\let\endproof\relax
%\renewcommand{\citedash}{--}
\usepackage[square, comma, numbers]{natbib}
\setlength{\bibsep}{10.0pt}
\def\bibfont{\small}

\usepackage[colorlinks,
            linkcolor=black,
            anchorcolor=black,
            citecolor=blue,
			urlcolor=black,
            bookmarks=true
            ]{hyperref}

\usepackage{url}
\usepackage{xcolor}
\usepackage[justification=justified,singlelinecheck=off,centerlast]{caption}
\newcommand{\term}[1]{\texttt{\small #1}}
\newcommand{\TODO}[2]{\textcolor{red}{\textbf{\small #1:} #2}} 	
\newcommand{\SOLVED}[2]{\textcolor{blue}{\textbf{\small #1:} #2}}
\newcommand{\csp}[1]{\texttt{\scriptsize #1}}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}



